Interpretable Vertebral Fracture Quantification via Anchor-Free Landmarks Localization

Vertebral body compression fractures are early signs of osteoporosis. Though these fractures are visible on Computed Tomography (CT) images, they are frequently missed by radiologists in clinical settings. Prior research on automatic methods of vertebral fracture classification proves its reliable quality; however, existing methods provide hard-to-interpret outputs and sometimes fail to process cases with severe abnormalities such as highly pathological vertebrae or scoliosis. We propose a new two-step algorithm to localize the vertebral column in 3D CT images and then detect individual vertebrae and quantify fractures in 2D simultaneously. We train neural networks for both steps using a simple 6-keypoints based annotation scheme, which corresponds precisely to the current clinical recommendation. Our algorithm has no exclusion criteria, processes 3D CT in 2 seconds on a single GPU, and provides an interpretable and verifiable output. The method approaches expert-level performance and demonstrates state-of-the-art results in vertebrae 3D localization (the average error is 1 mm), vertebrae 2D detection (precision and recall are 0.99), and fracture identification (ROC AUC at the patient level is up to 0.96). Our anchor-free vertebra detection network shows excellent generalizability on a new domain by achieving ROC AUC 0.95, sensitivity 0.85, specificity 0.9 on a challenging VerSe dataset with many unseen vertebra types.

==> content/results_backup.tex <==
\newcommand{\lt}{\textless}

\section{Results}
\label{sec:results}

We report results obtained using 5-fold cross-validation. For every network we trained 5 experiments with different cross-validation splits in order to estimate mean and standard deviation for each score. 
To obtain patient-level predictions, we use the most severe fracture among all the vertebrae, which is equivalent to taking the minimal Genant score.
As we have multiple annotations per study, we also report the inter-expert variability. 

Unlike Lung-Cancer-500, VerSe has a publicly available division on train, validation and test. For this reason, we used the last two subsets for testing. %, while applying only one 5-fold split on the training sample.

\subsection{Spine localization}
\label{sec:spine-localization-results}

We report the localization quality of the first step of our method in Table \ref{tab:spine-localization-metrics}. 
Because most of the images from Lung-Cancer-500 (Section \ref{dataset:lung-cancer-500}) are fully covered by vertebrae, this dataset is not very challenging for the limits classification head.
Thus, in order to thoroughly evaluate the localization network, we use an additional dataset with annotated vertebrae centroids - VerSe-2020 (Section \ref{dataset:verse2020}).


\begin{table}[b!]
\caption{
    \label{tab:spine-localization-metrics}
    Spinal line localization metrics for Lung-Cancer-500 and VerSe-2020 datasets.
}
\begin{center}
\begin{tabular}{ccccc}
    \toprule 
%   \multirow{2}{*}{Method} 
   &Points RMSE(mm) & Limits MAE(mm) & Precision & Recall \\ 
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} 
    
    Cancer500 & 
        % \enskip 2 \times 2 \times 4 &
        \enskip .92 (.07) &
        \enskip .03 (.04) &
        \enskip 1.0 (.0) &
        1.0 (.0)  \\
        
    Cancer500 Private & 
        % \enskip 2 \times 2 \times 4 &
        \enskip .?? (.0?) &
        \enskip .?? (.0?) &
        \enskip ?.? (.?) &
        ?.? (.?)  \\

    VerSe val & 
        % \enskip 2 \times 2 \times 4 &
        \enskip 1.81 (.20) &
        \enskip 19.23 (3.42) &
        \enskip .96 (.01) &
        .99 (.01) \\
        
    VerSe val Private & 
        % \enskip 2 \times 2 \times 4 &
        \enskip .?? (.0?) &
        \enskip .?? (.0?) &
        \enskip ?.? (.?) &
        ?.? (.?)  \\

    VerSe test & 
        % \enskip 2 \times 2 \times 4 &
        \enskip 1.72 (.17) &
        \enskip 18.76 (2.59) &
        \enskip .96 (.01) &
        .99 (.01) \\
        
    VerSe test Private & 
        % \enskip 2 \times 2 \times 4 &
        \enskip .?? (.0?) &
        \enskip .?? (.0?) &
        \enskip ?.? (.?) &
        ?.? (.?)  \\
    
    % # The previous version
    % Cancer-500 & 
    %     % \enskip 2 \times 2 \times 4 &
    %     \enskip 1.607 (.020) &
    %     \enskip .096 (.131) &
    %     \enskip 1.0 (.0) &
    %     1.0 (.0)  \\

    % VerSe val & 
    %     % \enskip 2 \times 2 \times 4 &
    %     \enskip .910 (.026) &
    %     \enskip 19.17 (7.04) &
    %     \enskip .978 (.015) &
    %     .975 (.009) \\

    % VerSe test & 
    %     % \enskip 2 \times 2 \times 4 &
    %     \enskip .991 (.067) &
    %     \enskip 25.14 (4.56) &
    %     \enskip .972 (.013) &
    %     .973 (.009) \\
        
    % # the end of the previous version
        
    % VerSe val &
    %     \enskip 3 \times 3 \times 3 &
    %     \enskip 1.29 (.05) &
    %     \enskip 24.0 (5.3) &
    %     \enskip .982 (.003) &
    %     .959 (.003) \\
    
    % VerSe test &
    %     \enskip 3 \times 3 \times 3 &
    %     \enskip 1.53 (.16) &
    %     \enskip 27.7 (1.2) &
    %     \enskip .975 (.003) &
    %     .957 (.004) \\
        
    \bottomrule
\end{tabular}
\end{center}
\end{table}

The difference in the RMSE metric between the two datasets can be 
%partly 
explained by the fact that the images of VerSe are much more diverse than those of Lung-Cancer-500. 
Nevertheless, given the input voxel size of $2\times 2\times 4mm$, the results on both the datasets suggest that the model's performance is close to maximal.

%Moreover, it is worth mentioning that, strictly speaking, the centers calculated from Genant segments may not coincide with the actual centers of the vertebral bodies. As a consequence, the localization problems on the datasets may be considered as two slightly different tasks. 

Moreover, as mentioned in Section \ref{dataset:verse2020}, the vertebrae near image limits are sometimes lacking annotation (Fig. \ref{fig:verse}). We argue that this is the main cause of such a large \textit{Limits MAE} in Tab. \ref{tab:spine-localization-metrics}. For this reason, we additionally extrapolate the predictions by 2cm at both limits, leaving the second network with more potential vertebrae to detect. Surprisingly, this increased the overall recall of the pipeline, but doesn't deteriorate the precision significantly (Tab. \ref{tab:detection-metrics}).


\subsection{Vertebrae detection and severity classification}

\subsubsection{Cross-validation on Cancer500}
In order to calculate vertebrae-level metrics a matching procedure of predicted and real vertebrae is required. For Cancer500 we use an NMS-inspired approach by calculating a closeness function (namely \todo{BIoU}) between each $(prediction, target)$ pair. 
For VerSe another matching procedure is required, given the fact that the annotation represents vertebrae centers. Similarly to \citep{verse1} we use the Euclidean distance between centers as a closeness function with a threshold of 20 mm.
All pairs with a closeness smaller than a given threshold are discarded. For the remaining pairs, for each $target$ we select the closest corresponding $prediction$. This way all unmatched targets are considered false negatives (FN) and all unmatched predictions - false positives (FP). Table. \ref{tab:detection-metrics} shows vertebrae detection metrics averaged by patients as well as by vertebrae.

\begin{table}
\caption{
    \label{tab:detection-metrics}
    Vertebrae detection performance. The first three rows are calculated for the LungCancer500 dataset.
}
\begin{center}
\begin{tabular}{lccc}
    \toprule 
    & \multicolumn{2}{c}{Detection}  \\
%   \multirow{2}{*}{Method} 
   & Precision & Recall \\ % & Types Accuracy \\ 
    % \cmidrule(lr){1-1}
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} %\cmidrule(lr){4-4}
    
    Anchor-Boxes &
        \enskip .995 (.001) &
        \enskip .953 (.001) \\
        %-- \\
    
    Ours Public & 
        \enskip .995 (.001) &
        \enskip .987 (.001) \\
        
     \todo{Ours Private} & 
        \enskip .99? (.00?) &
        \enskip .99? (.00?) \\
        %-- \\
    
    % + Types-1 & 
    %     \enskip .993 (.001) &
    %     \enskip .991 (.001) &
    %     .81 (.03) \\
    
    % + Types-41 &
    %     \enskip .992 (.002) &
    %     \enskip .991 (.002) &
    %     .91 (.02) \\

    % + T-41 newMLE &
    %     \enskip .992 (.002) &
    %     \enskip .991 (.002) &
    %     .93 (.01) \\
    
    Experts & 
        \enskip .999 (.001) &
        \enskip .994 (.001) \\ 
        %1.0 \\
    
    \arrayrulecolor{black!30}\cmidrule(lr){1-3}
    \arrayrulecolor{black}
    
    Ours (VerSe) &
        \enskip .947 &
        \enskip .886 \\

    Ours (VerSe ext) &
        \enskip .935 &
        \enskip .951 \\
    
    % Anchors & 
    %     \enskip .995 (.001) &
    %     \enskip .953 (.001) &
    %     -- \\

    % JustPoints & 
    %     \enskip .995 (.001) &
    %     \enskip .987 (.001) &
    %     -- \\

    % KerSize=3 & 
    %     \enskip .993 (.001) &
    %     \enskip .991 (.001) &
    %     .79 (.04) \\

    % KerSize=1 & 
    %     \enskip .993 (.001) &
    %     \enskip .991 (.001) &
    %     .81 (.03) \\
        
    % 41 channels &
    %     \enskip .993 (.001) &
    %     \enskip .991 (.001) &
    %     .90 (.02) \\

    % 41chnls-v2 &
    %     \enskip .992 (.002) &
    %     \enskip .991 (.002) &
    %     .91 (.02) \\
    
    % Experts & 
    %     \enskip .999 (.001) &
    %     \enskip .994 (.001) & 
    %     1.0 \\
    \bottomrule
\end{tabular}
\end{center}
\end{table}

% \todo{As we find best sequence of labels, usually if we misclassify one vertebra we misclassify all other vertebrae and vice versa. So, accuracy of about 80\% means that in every fifth image our algorithm mislabel types, and in all cases this mislabeling has a shift of just one vertebrae.}

To analyze the performance of vertebrae fracture severity classification, we report metrics for two threshold values of $G$ following the radiological definition of severity \citep{genant}, see Tab. \ref{tab:severity-metrics}. We assume that the most relevant problem for chest CT is the identification of at least Moderate fractures ($G\le0.74$) as healthy vertebrae in the thoracic spine are wedged, so normal variation can be misclassified as a Mild fracture ($0.74<G\le0.8$) \citep{lenchik2004diagnosis}. 


% \begin{table}
% \caption{
%     \label{tab:severity-metrics}
%     Binary classification metrics for various grades of fractures: at least \textit{Mild} ($G \le 0.8$) and at least \textit{Moderate} ($G \le 0.74)$.
%     All numbers are given as mean (std).
%     Columns with white background denote vertebrae-level predictions, the ones with grey background - patient-level predictions.
% }
% \begin{center}
% \begin{tabular}{ccrarara}
%     \toprule 

%     Grade & $G$ by & \multicolumn{2}{c}{ROC AUC} & \multicolumn{2}{c}{Specificity} &
%     \multicolumn{2}{c}{Sensitivity} \\ 
%     \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}

% % 	Patient				Vertebra		
% % 01vs23	AUC	Specificity	Sensitivity		AUC	Specificity	Sensitivity

%   \multirow{6}{*}{Mild} &
%   Anchors 
%   &\enskip
%   % AUC
%         .889 (.004) & \enskip
%         .892 (.016) & \enskip
%     %Specificity
%         .949 (.006) & \enskip
%         .75 (.07) & \enskip
%     %Sensitivity
%         .55 (.02) & \enskip
%         .84 (.04) \\

%   &JustPoints
%   &\enskip
%   % AUC
%         .913 (.003) & \enskip
%         .897 (.008) & \enskip
%     %Specificity
%         .960 (.005) & \enskip
%         .81 (.06) & \enskip
%     %Sensitivity
%         .607 (.012) & \enskip
%         .822 (.006) \\

%   &KerSize=3
%   &\enskip
%   % AUC
%         .914 (.006) & \enskip
%         .899 (.013)   & \enskip
%     %Specificity
%         .962 (.003)   & \enskip
%         .78 (.03)   & \enskip
%     %Sensitivity
%         .61 (.02)   & \enskip
%         .83 (.02)  \\

%   &KerSize=1
%   &\enskip
%   % AUC
%         .909 (.005) & \enskip
%         .90 (.02) & \enskip
%     %Specificity
%         .959 (.002) & \enskip
%         .79 (.04) & \enskip
%     %Sensitivity
%         .602 (.009) & \enskip
%         .84 (.03) \\
    
%   &41 channels
%   &\enskip
%   % AUC
%         .909 (.006) & \enskip
%         .85 (.03) & \enskip
%     %Specificity
%         .967 (.004) & \enskip
%         .72 (.03) & \enskip
%     %Sensitivity
%         .58 (.02) & \enskip
%         .82 (.03) \\
    
%     &Experts \quad &
%     % AUC
%         .909 (.005) &
%         .90 (.03) & 
%     %Specificity
%         .914 (.006) &
%         .62 (.03) & 
%     %Sensitivity
%         .722 (.014) &
%         .925 (.016) \\ \hline % \cmidrule(lr){1-7}

    
%     % \rowcolor{gray}
%     % \cellcolor{white}

%     \multirow{6}{*}{Moderate\;} &
%     Anchors 
%     &\enskip
%     % AUC
%         .945 (.004) & \enskip
%         .938 (.007) & \enskip
%     %Specificity
%         .990 (.003) & \enskip
%         .95 (.02) & \enskip
%     %Sensitivity
%         .58 (.02) & \enskip
%         .75 (.03) \\

%     &JustPoints
%     &\enskip
%     % AUC
%         .955 (.006) & \enskip
%         .954 (.007) & \enskip
%     %Specificity
%         .990 (.002) & \enskip
%         .962 (.016) & \enskip
%     %Sensitivity
%         .619 (.006) & \enskip
%         .804 (.015) \\

%     &KerSize=3 \quad &
%     % AUC
%         .959 (.006) &
%         .947 (.011) &
%     %Specificity
%         .989 (.001) &
%         .948 (.010) &
%      %Sensitivity
%         .61 (.02) &
%         .77 (.03) \\

%   &KerSize=1
%   &\enskip
%   % AUC
%         .956 (.004) & \enskip
%         .949 (.001) & \enskip
%     %Specificity
%         .989 (.001) & \enskip
%         .95 (.03) & \enskip
%     %Sensitivity
%         .62 (.02) & \enskip
%         .793 (.017) \\

%   &41 channels
%   &\enskip
%   % AUC
%         .953 (.007) & \enskip
%         .938 (.015) & \enskip
%     %Specificity
%         .987 (.001) & \enskip
%         .94 (.02) & \enskip
%     %Sensitivity
%         .63 (.02) & \enskip
%         .76 (.03) \\

        
%     &Experts \quad &\
%     % AUC
%         .974 (.003) &
%         .950 (.010) & 
%     %Specificity
%         .974 (.004) &
%         .85 (.04) &
%      %Sensitivity
%         .79 (.04) & 
%         .90 (.04) \\ % \cmidrule(lr){1-7}
    
%     \bottomrule
% \end{tabular}
% \end{center}
% \end{table}


% \begin{table}
% \caption{
%     \label{tab:severity-metrics2}
%     Binary classification metrics for various grades of fractures: at least \textit{Mild} ($G \le 0.8$) and at least \textit{Moderate} ($G \le 0.74)$.
%     All numbers are given as mean (std).
%     Columns with white background denote vertebrae-level predictions, the ones with grey background - patient-level predictions.
% }

% \begin{center}
% \begin{tabular}{crrrr}
%     \toprule 

%     $G$ by & ROC-AUC & Specificity & 
%     Sensitivity & Accuracy \\ 
%     \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}

% % 	Patient				Vertebra		
% % 01vs23	AUC	Specificity	Sensitivity		AUC	Specificity	Sensitivity
    
%     \multicolumn{1-5}{c}{{Mild}}
%     \cmidrule(lr){1-5}

%   Anchors 
%   &
%   % AUC
%         .89 (.01) & 
%     %Specificity
%         .95 (.01) & 
%     %Sensitivity
%         .55 (.02) & 
%     %Types accuracy
%         -- \\

%   JustPoints
%   &
%   % AUC
%         .91 (.01) & 
%     %Specificity
%         .96 ( .01) & 
%     %Sensitivity
%         .61 (.01) & 
%     %Types accuracy
%         -- \\

%   KerSize=3
%   &
%   % AUC
%         .91 (.01) & 
%     %Specificity
%         .96 (.01)   & 
%     %Sensitivity
%         .61 (.02)   & 
%     %Types accuracy
%         -- \\

%   KerSize=1
%   &
%   % AUC
%         .91 (.01) & 
%     %Specificity
%         .96 (.01) & 
%     %Sensitivity
%         .60 (.01) & 
%     %Types accuracy
%         -- \\
    
%   41 channels
%   &
%   % AUC
%         .91 (.01) & 
%     %Specificity
%         .97 (.01) & 
%     %Sensitivity
%         .58 (.02) & 
%     %Types accuracy
%         -- \\
    
%     Experts  &
%     % AUC
%         .91 ( .01) &
%     %Specificity
%         .91 ( .01) &
%     %Sensitivity
%         .72 (.01) &
%     %Types accuracy
%         -- \\
%     \hline % \cmidrule(lr){1-7}
    
%     % \rowcolor{gray}
%     % \cellcolor{white}

%     \multicolumn(lr){1-5}{Moderate} 
%     \cmi
    
%     Anchors 
%     &\enskip
%     % AUC
%         .95 (\lt .01) & \enskip
%     %Specificity
%         .99 (\lt .01) & \enskip
%     %Sensitivity
%         .58 (.02) & \enskip
%     %Types accuracy
%         -- \\

%     &JustPoints
%     &\enskip
%     % AUC
%         .96 (\lt .01) & \enskip
%     %Specificity
%         .99 (\lt .01) & \enskip
%     %Sensitivity
%         .62 (\lt .01) & \enskip
%     %Types accuracy
%         -- \\

%     &KerSize=3 \quad &
%     % AUC
%         .96 (\lt .01) &
%     %Specificity
%         .99 (\lt .01) &
%      %Sensitivity
%         .61 (.02) &
%     %Types accuracy
%         -- \\

%   &KerSize=1
%   &\enskip
%   % AUC
%         .96 (\lt .01) & \enskip
%     %Specificity
%         .99 (\lt .01) & \enskip
%     %Sensitivity
%         .62 (.02) & \enskip
%     %Types accuracy
%         -- \\

%   &41 channels
%   &\enskip
%   % AUC
%         .95 (\lt .01) & \enskip
%     %Specificity
%         .99 (\lt .01) & \enskip
%     %Sensitivity
%         .63 (.02) & \enskip
%     %Types accuracy
%         -- \\

%     &Experts \quad &\
%     % AUC
%         .97 (\lt .01) &
%     %Specificity
%         .97 (\lt .01) &
%      %Sensitivity
%         .79 (.04) & 
%     %Types accuracy
%         -- \\

%     \bottomrule
% \end{tabular}
% \end{center}
% \end{table}



\begin{table}
\caption{
    \label{tab:severity-metrics}
    Binary classification metrics for various grades of fractures: at least \textit{Mild} ($G \le 0.8$) and at least \textit{Moderate} ($G \le 0.74)$.
    All numbers are given as mean (std).
    Columns with white background denote vertebrae-level predictions, the ones with grey background - patient-level predictions. First three rows report the results for the Cancer500 dataset.
}
\begin{center}
\setlength\tabcolsep{0.4em}
\begin{tabular}{l|r >{\columncolor[gray]{0.93}}r | r >{\columncolor[gray]{0.93}}r | r >{\columncolor[gray]{0.93}}r}
    \toprule 

% 	Patient				Vertebra		
% 01vs23	AUC	Specificity	Sensitivity		AUC	Specificity	Sensitivity

    \multicolumn{7}{c}{\textit{Mild}} \\
    \cmidrule(lr){1-7}

    $G$ by & \multicolumn{2}{c|}{ROC AUC} & \multicolumn{2}{c|}{Specificity} &
    \multicolumn{2}{c}{Sensitivity} \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
    
    Anchor-Boxes
    &
    % AUC
        .89 (.01) & 
        .89 (.02) & 
    %Specificity
        .95 (.01) & 
        .75 (.07) & 
    %Sensitivity
        .55 (.02) & 
        .84 (.04) \\

    Ours
    &
    % AUC
        .91 (.01) & 
        .90 (.01) & 
    %Specificity
        .96 (.01) & 
        .81 (.06) & 
    %Sensitivity
        .61 (.01) & 
        .82 (.01) \\

%   + Types-1
%   &
%   % AUC
%         .91 (.01) & 
%         .90 (.01)   & 
%     %Specificity
%         .96 (.01)   & 
%         .78 (.03)   & 
%     %Sensitivity
%         .61 (.02)   & 
%         .83 (.02) \\

% %   KerSize=1
% %   &
% %   % AUC
% %         .91 (.01) & 
% %         .90 (.02) & 
% %     %Specificity
% %         .96 (.01) & 
% %         .79 (.04) & 
% %     %Sensitivity
% %         .60 (.01) & 
% %         .84 (.03) \\
    
% %   41 channels
% %   &
% %   % AUC
% %         .91 (.01) &
% %         .85 (.03) & 
% %     %Specificity
% %         .97 (.01) & 
% %         .72 (.03) & 
% %     %Sensitivity
% %         .58 (.02) & 
% %         .82 (.03) \\

%   + Types-41
%   &
%   % AUC
%         .91 (.01) &
%         .88 (.02) & 
%     %Specificity
%         .95 (.01) & 
%         .78 (.03) & 
%     %Sensitivity
%         .60 (.01) & 
%         .82 (.01) \\
    
    Experts  &
    % AUC
        .91 (.01) &
        .90 (.03) & 
    %Specificity
        .91 (.01) &
        .62 (.03) & 
    %Sensitivity
        .72 (.01) &
        .93 (.02) \\
    %\hline % \cmidrule(lr){1-7}
    % \midrule
    
    \arrayrulecolor{black!30}\cmidrule(lr){1-7}
    \arrayrulecolor{black}
    
    Ours (VerSe)
    &
    % AUC
        .88 (.01) & 
        .88 (.01) & 
    %Specificity
        .94 (.01) & 
        .72 (.04) & 
    %Sensitivity
        .66 (.01) & 
        .89 (.01) \\

    
    \cmidrule(lr){1-7} 
    
    % \rowcolor{gray}
    % \cellcolor{white}

    \multicolumn{7}{c}{\textit{Moderate}} \\
    \cmidrule(lr){1-7} 

    % $G$ by & \multicolumn{2}{c}{ROC AUC} & \multicolumn{2}{c}{Specificity} &
    % \multicolumn{2}{c}{Sensitivity} & Accuracy\\ 
    % \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} 
    
    Anchor-Boxes
    &
    % AUC
        .95 (.01) & 
        .94 (.01) & 
    %Specificity
        .99 (.01) & 
        .95 (.02) & 
    %Sensitivity
        .58 (.02) & 
        .75 (.03) \\

    Ours
    &
    % AUC
        .96 (.01) & 
        .95 (.01) & 
    %Specificity
        .99 (.01) & 
        .96 (.02) & 
    %Sensitivity
        .62 (.01) & 
        .81 (.02) \\

%     + Types-1  &
%     % AUC
%         .96 (.01) &
%         .95 (.01) &
%     %Specificity
%         .99 (.01) &
%         .95 (.01) &
%      %Sensitivity
%         .61 (.02) &
%         .77 (.03) \\

% %   KerSize=1
% %   &
% %   % AUC
% %         .96 (.01) & 
% %         .95 (.01) & 
% %     %Specificity
% %         .99 (.01) & 
% %         .95 (.03) & 
% %     %Sensitivity
% %         .62 (.02) & 
% %         .79 (.02) \\

% %   41 channels
% %   &
% %   % AUC
% %         .95 (.01) & 
% %         .94 (.01) & 
% %     %Specificity
% %         .99 (.01) & 
% %         .94 (.02) & 
% %     %Sensitivity
% %         .63 (.02) & 
% %         .76 (.03) \\

%   + Types-41
%   &
%   % AUC
%         .96 (.01) &
%         .95 (.01) & 
%     %Specificity
%         .99 (.01) & 
%         .95 (.03) & 
%     %Sensitivity
%         .64 (.03) & 
%         .77 (.03) \\

    Experts  &\
    % AUC
        .97 (.01) &
        .95 (.01) & 
    %Specificity
        .97 (.01) &
        .85 (.04) &
     %Sensitivity
        .79 (.04) & 
        .90 (.04) \\
    
    \arrayrulecolor{black!30}\cmidrule(lr){1-7}
    \arrayrulecolor{black}
    
    Ours (VerSe)
    &
    % AUC
        .96 (.01) & 
        .94 (.01) & 
    %Specificity
        .97 (.01) & 
        .85 (.02) & 
    %Sensitivity
        .73 (.05) & 
        .90 (.01) \\

    
    \bottomrule
\end{tabular}
\end{center}
\end{table}


Moreover, we analyze the generalizability of our approach by evaluating the model on the VerSe dataset, which contains additional annotations regarding the fracture severity of each vertebra. In this experiment we only trained the spine localization network on VerSe and reused the vertebrae detection network (trained on Cancer500) \textit{as is}, without any additional tuning. The results are shown in the last rows of Tables \ref{tab:detection-metrics} and \ref{tab:severity-metrics}. Note the minimal drop in classification performance.

It is important to note that the results for the VerSe dataset from Tab. \ref{tab:detection-metrics} are underestimated, especially the precision. This significant drop in quality is due to lacking annotations for vertebrae near images' edges. Fig. \ref{fig:verse} shows several examples with such "false positives". According to our calculations about $95\%$ of FPs are due to such partially annotated cases.

\begin{figure}
    \begin{center}
      \includegraphics[width=1.\linewidth]{figures/verse-limits.png}
      \caption{
        Several examples of "false positives" on the VerSe dataset in sagittal and coronal projections. The annotated vertebrae are marked with orange stars, the predicted ones - with blue circles. Note the missing annotations for "border" vertebrae: near image borders (a-b), vertebral column borders (c-f)
        \label{fig:verse}
      }
    \end{center}
\end{figure}

Overall, the obtained results are close to human-level performance on our dataset and comparable with other works. Similar values of ROC AUC were obtained at vertebra ($0.88$ \citep{valentinitsch2019opportunistic}, $0.93$ \citep{nicolaes-segmentation}) and patient levels ($0.92$ \citep{tomita-rnn}). 


